Accurate, scalable, and efficient Bayesian optimal experimental design with derivative-informed neural operators

We consider optimal experimental design (OED) problems in selecting the most informative observation sensors to estimate model parameters in a Bayesian framework. Such problems are computationally prohibitive when the parameter-to-observable (PtO) map is expensive to evaluate, the parameters are high-dimensional, and the optimization for sensor selection is combinatorial and high-dimensional. To address these challenges, we develop an accurate, scalable, and efficient computational framework based on derivative-informed neural operators (DINO). We propose to use derivative-informed dimension reduction to reduce the parameter dimensions, based on which we train DINO with derivative information as an accurate and efficient surrogate for the PtO map and its derivative. Moreover, we derive DINO-enabled efficient formulations in computing the maximum a posteriori (MAP) point, the eigenvalues of approximate posterior covariance, and three commonly used optimality criteria for the OED problems. Furthermore, we provide detailed error analysis for the approximations of the MAP point, the eigenvalues, and the optimality criteria. We also propose a modified swapping greedy algorithm for the sensor selection optimization and demonstrate that the proposed computational framework is scalable to preserve the accuracy for increasing parameter dimensions and achieves high computational efficiency, with an over 1000$\times$ speedup accounting for both offline construction and online evaluation costs, compared to high-fidelity Bayesian OED solutions for a three-dimensional nonlinear convection-diffusion-reaction example with tens of thousands of parameters.

==> analysis.tex <==
\section{Error analysis}

This section analyzes the error in our proposed method for MAP point estimation and the eigenvalues of the corresponding Gauss-Newton Hessian at the MAP point. We introduce assumptions to address challenges in non-convex optimization and utilizing neural network forward models. These assumptions form the basis for bounding the errors in both the MAP point estimation and the corresponding eigenvalue calculations. We further validate these assumptions in the numerical results presented in Section \ref{sec:numerical}. As part of our error analysis, we use these assumptions to verify the convergence of the MAP point from the proposed method. We also verify the convergence of the eigenvalues under these assumptions.

\label{sec:ErrorAnalysis}
\subsection{Approximation error of the MAP point}
\label{sec:ErrorAnalysis-map}
Let the objective function in \eqref{eq:MAP} for the high-fidelity MAP point be denoted as 
\begin{equation}\label{eq:objMAP}
    L(\bsm) = \frac{1}{2}||\bsy- F_\xi(\bsm)||^2_{\Gamma_\text{noise}^{-1}}+\frac{1}{2}||\bsm-\bsm_\text{prior}||^2_{\Gamma_\text{prior}^{-1}}
\end{equation}
for any design $\xi$ and data $\bsy$. Let $\hat{F}_\xi$ denote the neural network approximation of the forward map $F_\xi$ given in \eqref{eq:Fnn}. Let $\hat{L}$ denote the corresponding objective function in \eqref{eq:rMAP}, which can be equivalently written as a function of the high-fidelity parameter as 
\begin{equation}\label{eq:hatobjMAP}
    \hat{L}(\bsm) = \frac{1}{2}||\bsy- \hat{F}_\xi(\bsm)||^2_{\Gamma_\text{noise}^{-1}}+\frac{1}{2}||P_r(\bsm) - \bsm_\text{prior}||^2_{\Gamma_\text{prior}^{-1}},
\end{equation} 
where $P_r$ represents the linear projection operator defined as in \eqref{eq:ias} or \eqref{eq:kle}. Moreover, we denote the MAP point obtained from the high-fidelity optimization problem \eqref{eq:MAP} as $\bsm^*$ and the MAP point obtained from the projected optimization problem \eqref{eq:rMAP} as $\hat{\bsm}^*$, which satisfy the stationary conditions 
\begin{equation}\label{eq:staionaryM}
  0 = \nabla_\bsm L(\bsm^*) =  - (\bsy - F_\xi(\bsm^*))^T\Gamma_\text{noise}^{-1}\nabla_\bsm F_\xi(\bsm^*) + \Gamma_\text{prior}^{-1} (\bsm^* - \bsm_\text{prior})
\end{equation}
and 
\begin{equation}\label{eq:staionaryMhat}
  0 = \nabla_\bsm \hat{L}(\hat{\bsm}^*) = - (\bsy - \hat{F}_\xi(\hat{\bsm}^*))^T\Gamma_\text{noise}^{-1}\nabla_\bsm \hat{F}_\xi(\hat{\bsm}^*) + \Gamma_\text{prior}^{-1} (P_r(\hat{\bsm}^*) - \bsm_\text{prior}),
\end{equation}
respectively. To bound the approximation error of the MAP point obtained in \eqref{eq:rMAP} and the eigenvalues obtained in \eqref{eq:rEig} by the neural network approximation of the forward map,
we make the following assumptions on the objective function $L$ and $\hat{L}$, 
the approximation error of the forward map and its Jacobian by DINO, the dimension reduction error of the MAP point. We use $||\cdot||$ to denote the Euclidean norm for vectors and the Frobenius norm for matrices. 

\begin{assumption}\label{ass:assumptions}
Let $\bsm^*$ and $\hat{\bsm}^*$ be the MAP points obtained from the high-fidelity optimization problem \eqref{eq:MAP} and the projected optimization problem \eqref{eq:rMAP}, satisfying $\nabla_\bsm L(\bsm^*) = 0$ and $\nabla_\bsm \hat{L}(\hat{\bsm}^*) = 0$,  respectively.
    \begin{itemize}
        \item[A1] We assume that the gradients  $\nabla_\bsm L$ and $\nabla_\bsm \hat{L}$ allow convergent Taylor expansion around $\bsm^*$ and $\hat{\bsm}^*$\label{ass:ass-1}, 
  \begin{equation}\label{eq:Taylor1}
    \nabla_\bsm L(\bsm) = \nabla_\bsm L(\bsm^*) + \nabla_\bsm^2 L(\bsm^*)(\bsm - \bsm^*) + \delta(\bsm) (\bsm - \bsm^*),
  \end{equation}
  for $\bsm$ such that $||\bsm - \bsm^*|| \leq R_m$, and 
  \begin{equation}\label{eq:Taylor2}
    \nabla_\bsm \hat{L}(\bsm) = \nabla_\bsm \hat{L}(\hat{\bsm}^*) +\nabla_\bsm^2 \hat{L}(\hat{\bsm}^*)(\bsm - \hat{\bsm}^*) + \hat{\delta}(\bsm) (\bsm - \hat{\bsm}^*),
  \end{equation}
  for $\bsm$ such that $||\bsm - \hat{\bsm}^*|| \leq R_m$, for some radius $R_m$, where $\delta(\bsm) \in \mathbb{R}^{d_m \times d_m}$ and $\hat{\delta}(\bsm) \in \mathbb{R}^{d_m \times d_m}$ satisfy $\lim_{\bsm \to \bsm^*}||\delta(\bsm)|| = 0$ and $\lim_{\bsm \to \hat{\bsm}^*}||\hat{\delta}(\bsm)|| = 0$, respectively.
 In addition, we assume that
 \begin{equation}\label{eq:lowerbound}
     ||(\nabla_\bsm^2 \hat{L}(\hat{\bsm}^*) + \nabla_\bsm^2 L(\bsm^*)) (\bsm^* - \hat{\bsm}^*) + (\hat{\delta}(\bsm^*) + \delta(\hat{\bsm}^*)) (\bsm^* - \hat{\bsm}^*)|| \geq c_h ||(\bsm^* - \hat{\bsm}^*)||
 \end{equation}
 for some constant $c_h > 0$. Note that this is satisfied under the stronger assumption that  
 the Hessian $\nabla_{\bsm}^2 L(\bsm^*)$ and $\nabla_\bsm^2 \hat{L}(\hat{\bsm}^*)$ at the MAP points are positive definite with the smallest eigenvalues $\lambda^*_{\text{min}} \geq c_\lambda > 0$ and $\hat{\lambda}^*_{\text{min}} \geq c_\lambda > 0$ for some constant $c_\lambda$, and $||\hat{\delta}(\bsm^*)|| \leq c_\delta$ and $||\delta(\hat{\bsm}^*)|| \leq c_\delta$ for some $c_\delta < c_\lambda$, which leads to $c_h \geq 2(c_\lambda - c_\delta) > 0$ for $c_h$ in \eqref{eq:lowerbound}. 
        
        \item[A2] Moreover, we assume that the forward map $F_\xi$ and its Jacobian $\nabla_\bsm F_\xi$ are bounded and well approximated by the bounded neural network approximation $\hat{F}_\xi$ and its Jacobian $\nabla_\bsm \hat{F}_\xi$ in the sense that there exist small positive constants $\varepsilon_1$ and $\varepsilon_2$ such that\label{ass:ass-2}
  \begin{equation}\label{eq:approxFJ}
    ||F_\xi(\bsm) - \hat{F}_\xi(\bsm)|| \leq \varepsilon_1 \quad \text{ and } \quad ||\nabla_\bsm F_\xi(\bsm) - \nabla_\bsm \hat{F}_\xi(\bsm)|| \leq \varepsilon_2
  \end{equation}
  for $\bsm$ such that $||\bsm - \bsm^*|| \leq R_m$ and $||\bsm - \hat{\bsm}^*|| \leq R_m$, in particular for $\bsm = \bsm^*$ and $\bsm = \hat{\bsm}^*$.


    \item[A3] Furthermore, we assume that there exists a bound $\varepsilon_3 > 0$ such that the error of the linear projection defined in \eqref{eq:ias} and \eqref{eq:kle} satisfy\label{ass:ass-3}
  \begin{equation}
    ||\Gamma_\text{prior}^{-1}(P_r(\bsm^*) - \bsm^*)|| \leq \varepsilon_3.
  \end{equation}
    \end{itemize}
\end{assumption}

We remark that assumption A1 is mild and holds true for linear or linearized inverse problems where the forward map $F_\xi(\bsm) = A \, \bsm $, linear with respect to the parameter, in which case $\delta(\bsm) = 0$ and $\hat{\delta}(\bsm) = 0$, and the Hessian $\nabla_\bsm^2 L(\bsm^*) = A^T \Gamma_{\text{noise}}^{-1} A + \Gamma_{\text{prior}}^{-1}$  is positive definite. However, it may not be true for highly nonlinear inverse problems such that the objective function $L$ and $\hat{L}$ become highly nonconvex and allow multiple local minima far away from each other. Assumption A2 is reasonable since the neural network approximation $\hat{F}_\xi$ is trained for both the function and its Jacobian in the DINO framework. Assumption A3 holds true for problems with intrinsic low-dimensionality of the input parameter, or the forward map lives in an intrinsically low-dimensional manifold of the parameter space. We will 
numerically investigate the decay of the approximation errors with increasing training data to demonstrate A2 and the dimension reduction error with increasing reduced dimension to demonstrate A3 in detail in Section \ref{sec:numerical}.

\begin{theorem}
\label{thm:1}
  Under Assumption \ref{ass:assumptions}, if $||\bsm^* - \hat{\bsm}^*|| \leq R_m$, we have the following error bound for the approximation of high-fidelity MAP point by the surrogate MAP point 
  \begin{equation}\label{eq:MAPbound}
    ||\bsm^* - \hat{\bsm}^*|| \leq c_1\varepsilon_1 + c_2\varepsilon_2 + c_3 \varepsilon_3,
  \end{equation}
  where $c_1 > 0, c_2>0,$ and $c_3 > 0$ are positive constants independent of $\varepsilon_1, \varepsilon_2, $ and $\varepsilon_3$.
\end{theorem}

\begin{proof}
  By A1 in Assumption \ref{ass:assumptions}, and $||\bsm^* - \hat{\bsm}^*|| \leq R_m$, we can evaluate the Taylor expansions \eqref{eq:Taylor1} and \eqref{eq:Taylor2} at $\bsm = \hat{\bsm}^*$ and $\bsm = \bsm^*$, respectively, and obtain 
\begin{equation}\label{eq:gradL}
    \nabla_\bsm L(\hat{\bsm}^*) = \nabla_\bsm^2 L(\bsm^*) (\hat{\bsm}^* - \bsm^*) + \delta(\hat{\bsm}^*)(\hat{\bsm}^* - \bsm^*)
\end{equation}
  and \begin{equation}\label{eq:gradhatL}
    \nabla_\bsm \hat{L}(\bsm^*) = \nabla_\bsm^2 \hat{L}(\hat{\bsm}^*) (\bsm^* - \hat{\bsm}^*) + \hat{\delta}(\bsm^*)(\bsm^* - \hat{\bsm}^*),
  \end{equation}
where we used the stationary conditions \eqref{eq:staionaryM} and \eqref{eq:staionaryMhat}. Subtracting \eqref{eq:gradL} from \eqref{eq:gradhatL}, we obtain
\begin{equation}\label{eq:hessgraddiff}
  \nabla_\bsm \hat{L}(\bsm^*) - \nabla_\bsm L(\hat{\bsm}^*) = (\nabla_\bsm^2 \hat{L}(\hat{\bsm}^*) + \nabla_\bsm^2 L(\bsm^*)) (\bsm^* - \hat{\bsm}^*) + (\delta(\hat{\bsm}^*) + \hat{\delta}(\bsm^*))(\bsm^* - \hat{\bsm}^*).
\end{equation}
By definition of $\hat{L}$ and $L$, we have for the left hand side of the above equation 
\begin{equation}\label{eq:gradLdiff}
  \begin{split}
  \nabla_\bsm \hat{L}(\bsm^*) - \nabla_\bsm L(\hat{\bsm}^*) & =  - (\bsy - \hat{F}_\xi(\bsm^*))^T\Gamma_\text{noise}^{-1}\nabla_\bsm \hat{F}_\xi(\bsm^*) + \Gamma_\text{prior}^{-1} (P_r(\bsm^*) - \bsm_\text{prior})\\
  & + (\bsy - F_\xi(\hat{\bsm}^*))^T\Gamma_\text{noise}^{-1}\nabla_\bsm F_\xi(\hat{\bsm}^*) - \Gamma_\text{prior}^{-1} (\hat{\bsm}^* - \bsm_\text{prior}).
  \end{split}
\end{equation}  
Let us consider the first term on the right hand side of the above equation. We have
\begin{equation}
  \begin{split}
    & - (\bsy - \hat{F}_\xi(\bsm^*))^T\Gamma_\text{noise}^{-1}\nabla_\bsm \hat{F}_\xi(\bsm^*) \\
  & = - (F(\bsm^*) - \hat{F}_\xi(\bsm^*))^T \Gamma_\text{noise}^{-1}\nabla_\bsm \hat{F}_\xi(\bsm^*) - (\bsy - F_\xi(\bsm^*))^T\Gamma_\text{noise}^{-1}\nabla_\bsm \hat{F}_\xi(\bsm^*)\\
  & = - A^T \Gamma_\text{noise}^{-1}\nabla_\bsm \hat{F}_\xi(\bsm^*) - (\bsy - F_\xi(\bsm^*))^T\Gamma_\text{noise}^{-1} (\nabla_\bsm \hat{F}_\xi(\bsm^*) - \nabla_\bsm F_\xi(\bsm^*)) \\
  & \quad - (\bsy - F_\xi(\bsm^*))^T\Gamma_\text{noise}^{-1}\nabla_\bsm F_\xi(\bsm^*)\\
  & = - A^T \Gamma_\text{noise}^{-1}\nabla_\bsm \hat{F}_\xi(\bsm^*) - (\bsy - F_\xi(\bsm^*))^T\Gamma_\text{noise}^{-1}B - \Gamma_{\text{prior}}^{-1} (\bsm^* - \bsm_\text{prior}),
  \end{split}
\end{equation}
where we added and subtracted $F_\xi(\bsm^*)$ in the first equality, added and subtracted $\nabla_\bsm F_\xi(\bsm^*)$ in the second equality while also setting $A = F(\bsm^*) - \hat{F}_\xi(\bsm^*)$, and used the stationary condition \eqref{eq:staionaryM} in the third equality while setting $B = \nabla_\bsm \hat{F}_\xi(\bsm^*) - \nabla_\bsm F_\xi(\bsm^*)$. 
% Note that $P_{r}(\hat{\bsm}^*) - \hat{\bsm}^* = 0$ because we solve $\hat{\bsm}^*$ in the reduced space. 
Similarly, we have for the third term in the right hand side of \eqref{eq:gradLdiff} by adding and subtracting $\hat{F}_\xi(\hat{\bsm}^*)$ and $\nabla_\bsm \hat{F}_\xi(\hat{\bsm}^*)$ and using the stationary condition \eqref{eq:staionaryMhat} to obtain 
\begin{equation}
  \begin{split}
  & (\bsy - F_\xi(\hat{\bsm}^*))^T\Gamma_\text{noise}^{-1}\nabla_\bsm F_\xi(\hat{\bsm}^*)\\
  & = C^T \Gamma_\text{noise}^{-1}\nabla_\bsm F_\xi(\hat{\bsm}^*) + (\bsy - \hat{F}_\xi(\hat{\bsm}^*))^T\Gamma_\text{noise}^{-1} D + \Gamma_{\text{prior}}^{-1} (P_r(\hat{\bsm}^*) - \bsm_\text{prior}),\\
  \end{split}
\end{equation}
where $C = \hat{F}_\xi(\hat{\bsm}^*) - F_\xi(\hat{\bsm}^*)$ and $D = \nabla_\bsm F_\xi(\hat{\bsm}^*)  - \nabla_\bsm \hat{F}_\xi(\hat{\bsm}^*)$. Substituting the above two equations into \eqref{eq:gradLdiff}, we obtain
\begin{equation}\label{eq:gradLdiff2}
  \begin{split}
  & \nabla_\bsm \hat{L}(\bsm^*) - \nabla_\bsm L(\hat{\bsm}^*) \\
  & = - A^T \Gamma_\text{noise}^{-1}\nabla_\bsm \hat{F}_\xi(\bsm^*) - (\bsy - F_\xi(\bsm^*))^T\Gamma_\text{noise}^{-1}B - \Gamma_{\text{prior}}^{-1} (\bsm^* - P_r(\bsm^*))\\
  & \quad + C^T \Gamma_\text{noise}^{-1}\nabla_\bsm F_\xi(\hat{\bsm}^*) + (\bsy - \hat{F}_\xi(\hat{\bsm}^*))^T\Gamma_\text{noise}^{-1} D + \Gamma_{\text{prior}}^{-1} (P_r(\hat{\bsm}^*) - \hat{\bsm}^*)\\
  & \leq \bar{c}_1 \varepsilon_1 + \bar{c}_2 \varepsilon_2 + \bar{c}_3\varepsilon_3,
  \end{split}
\end{equation}
where $\varepsilon_1$ and $\varepsilon_2$ are the bounds for the errors of the forward map and its Jacobian by the neural network approximation in \eqref{eq:approxFJ}, and $\varepsilon_3$ is the bound for the approximation error of the projection operator. Note that $\Gamma_{\text{prior}}^{-1} (P_r(\hat{\bsm}^*) - \hat{\bsm}^*) = 0$ in \eqref{eq:gradLdiff2} as $\hat{\bsm}^*$ is obtained in the projected subspace so that $P_r(\hat{\bsm}^*) = \hat{\bsm}^*$. The result follows by setting $\bar{c}_3 = 1$ and 
\begin{equation}
  \begin{split}
    \bar{c}_1 & = ||\Gamma_\text{noise}^{-1}||(||\nabla_\bsm \hat{F}_\xi(\bsm^*)|| + ||\nabla_\bsm F_\xi(\hat{\bsm}^*)||), \\
    \bar{c}_2 & = ||\Gamma_\text{noise}^{-1}||(2||\bsy|| + ||F_\xi(\bsm^*)|| + ||\hat{F}_\xi(\hat{\bsm}^*)||),
  \end{split}
\end{equation}
which are bounded by the assumption that the forward map and its Jacobian and their neural network approximations are bounded. For the right hand side of \eqref{eq:hessgraddiff}, we have the lower bound \eqref{eq:lowerbound} by assumption.
% For the right hand side of \eqref{eq:hessgraddiff}, we have
% \begin{equation}
%   |(\nabla_\bsm^2 \hat{L}(\hat{\bsm}^*) + \nabla_\bsm^2 L(\bsm^*)) (\bsm^* - \hat{\bsm}^*)| \geq c_\lambda ||\bsm^* - \hat{\bsm}^*||.
% \end{equation}
% Meanwhile, we have 
% \begin{equation}
%   \|(\delta(\hat{\bsm}^*) + \hat{\delta}(\bsm^*))(\bsm^* - \hat{\bsm}^*)\| \leq c_o ||\bsm^* - \hat{\bsm}^*||. 
% \end{equation}
% As a result, the absolute value of the right hand side of \eqref{eq:hessgraddiff} can be lower bounded by 
% \begin{equation}
%   |(\nabla_\bsm^2 \hat{L}(\hat{\bsm}^*) + \nabla_\bsm^2 L(\bsm^*)) (\bsm^* - \hat{\bsm}^*) + (\delta(\hat{\bsm}^*) + \hat{\delta}(\bsm^*))(\bsm^* - \hat{\bsm}^*)| \geq (c_\lambda-c_o)||\bsm^* - \hat{\bsm}^*||,
% \end{equation}
% when $2c_\lambda > c_o$. \textcolor{red}{After we check the $c_\lambda$, we decide $R_m$ to make $c_o \propto \|\hat{m}^* - m^*\|^2$ is smaller than $2c_\lambda$}. 
To this end, a combination of this lower bound and \eqref{eq:gradLdiff2} concludes by setting $c_i = \bar{c}_i/c_h$ with $i = 1, 2, 3$.
\end{proof}

\subsection{Approximation error of the eigenvalues}
\label{sec:ErrorAnalysis-eig}
We consider the approximation of the eigenvalues of the generalized eigenvalue problem \eqref{eq:disc-gen-eig} by those of the eigenvalue problem \eqref{eq:rEig} with neural network approximation of the forward map. 
\begin{theorem}
\label{thm:2}

Let $\lambda_i$, $i = 1, \dots, r$, denote the leading eigenvalues of the generalized eigenvalue problem \eqref{eq:disc-gen-eig}, and $\hat{\lambda}_i$, $i = 1, \dots, r$, denote those of the eigenvalue problem \eqref{eq:rEig}. Under Assumption \ref{ass:assumptions} and the assumption 
\begin{equation}\label{eq:Lipschitz}
    ||\nabla_\bsm F_\xi (\bsm^*) - \nabla_\bsm F_\xi(\hat{\bsm}^*)|| \leq L_F ||\bsm^* - \hat{\bsm}^*||
\end{equation}
for some Lipschitz constant $L_F$, we have 
\begin{equation}
    |\lambda_i - \hat{\lambda}_i| \leq \hat{c}_1 \varepsilon_1 + \hat{c}_2 \varepsilon_2 + \hat{c}_3 \varepsilon_3, \quad i = 1, \dots r, 
\end{equation}
for some constants $\hat{c}_1$, $\hat{c}_2$, and $\hat{c}_3$ independent of $\varepsilon_1$, $\varepsilon_2$, and $\varepsilon_3$.
\end{theorem}
\begin{proof}
    Let $H$ denote the prior-preconditioned Hessian of the misfit evaluated at the MAP point as
    \begin{equation}
        H = \Gamma_{\text{prior}}^{1/2} (\nabla_\bsm F_\xi(\bsm^*))^T \Gamma_{\text{noise}}^{-1} \nabla_\bsm F_\xi(\bsm^*) \Gamma_{\text{prior}}^{1/2},
    \end{equation}
then the eigenvalues of $H$, given by the eigenvalue problem   
\begin{equation}
    H \bsv_i = \lambda_i \bsv_i, \quad i = 1, \dots, r
\end{equation}
are the same as the eigenvalues of the generalized eigenvalue problem \eqref{eq:disc-gen-eig}, and the eigenvectors satisfy $\bsv_i = \Gamma_{\text{prior}}^{-1/2} \bsw_i$, $i = 1, \dots, r$. Let $\hat{H}$ denote the approximate prior-preconditioned Hessian of the misfit evaluated at the approximate MAP point as
\begin{equation}
    \hat{H} = \Gamma_{\text{prior}}^{1/2} (\nabla_\bsm \hat{F}_\xi(\hat{\bsm}^*))^T \Gamma_{\text{noise}}^{-1} \nabla_\bsm \hat{F}_\xi(\hat{\bsm}^*) \Gamma_{\text{prior}}^{1/2},
\end{equation}
then the eigenvalues of $\hat{H}$, given by the eigenvalue problem   
\begin{equation}
    \hat{H} \hat{\bsv}_i = \hat{\lambda}_i \hat{\bsv}_i, \quad i = 1, \dots, r
\end{equation}
are the same as the eigenvalues of the projected eigenvalue problem \eqref{eq:rEig}, and the eigenvectors $\hat{\bsv}_i = \Gamma_{\text{prior}}^{-1/2} 
 \Psi_\bsm \bsu_i$. This results from approximating the forward map with its approximate Jacobian $\nabla_\bsm \hat{F}_\xi $ given as in \eqref{eq:red-jac}. Let us first bound the Jacobians as 
 \begin{equation}
     ||\nabla_\bsm F_\xi(\bsm^*) - \nabla_\bsm \hat{F}_\xi(\hat{\bsm}^*)|| \leq ||\nabla_\bsm F_\xi(\bsm^*) - \nabla_\bsm F_\xi(\hat{\bsm}^*)|| + ||\nabla_\bsm F_\xi(\hat{\bsm}^*) - \nabla_\bsm \hat{F}_\xi(\hat{\bsm}^*)||
 \end{equation}
by a triangle inequality, which leads to the bound 
\begin{equation}\label{eq:JacBound}
     ||\nabla_\bsm F_\xi(\bsm^*) - \nabla_\bsm \hat{F}_\xi(\hat{\bsm}^*)|| \leq L_F ||\bsm^* - \hat{\bsm}^*|| + \varepsilon_2 \leq c_1 L_F \varepsilon_1 + (c_2 L_F + 1) \varepsilon_2 + c_3 L_F \varepsilon_3,
 \end{equation}
for which we used the Lipschitz continuity assumption in \eqref{eq:Lipschitz} and assumption \eqref{eq:approxFJ} in the first inequality and the bound \eqref{eq:MAPbound} for the MAP point approximation in the second inequality. Moreover, we have 
\begin{equation}\label{eq:HessBound}
    ||H - \hat{H}|| \leq c_H ||\nabla_\bsm F_\xi(\bsm^*) - \nabla_\bsm \hat{F}_\xi(\hat{\bsm}^*)||,
\end{equation}
with $c_H = ||\Gamma_{\text{prior}}|| \, ||\Gamma^{-1}_{\text{noise}}|| (||\nabla_\bsm F_\xi(\bsm^*)|| + ||\nabla_\bsm \hat{F}_\xi(\hat{\bsm}^*)||) $, 
for which we added and subtracted a term $\Gamma_{\text{prior}}^{1/2} (\nabla_\bsm \hat{F}_\xi(\hat{\bsm}^*))^T \Gamma_{\text{noise}}^{-1} \nabla_\bsm {F}_\xi({\bsm}^*) \Gamma_{\text{prior}}^{1/2}$ in $H - \hat{H}$. By Weyl's theorem \cite[Ch.\ 5.7]{bai2000templates} for the perturbation of Hermitian matrices, which both $H$ and $\hat{H}$ belong to, we have 
\begin{equation}
    |\lambda_i - \hat{\lambda}_i| \leq ||H - \hat{H}||_{\text{op}}, \quad i = 1, \dots, r,
\end{equation}
which concludes by using the bounds \eqref{eq:JacBound} and \eqref{eq:HessBound}, and the fact that the operator norm is smaller than the Frobenius norm, i.e., 
$||H - \hat{H}||_{\text{op}} \leq ||H - \hat{H}||$,
with constants 
\begin{equation}
    \hat{c}_1 = c_1 L_F c_H, \quad \hat{c}_2 = (c_2 L_F + 1) c_H, \quad \hat{c}_3 = c_3 L_F c_H.
\end{equation}
\end{proof}

\subsection{Approximation error of the optimality criteria}

